Method Towards CVPR 2021 Image Matching Challenge

This report describes Megvii-3D team's approach towards CVPR 2021 Image Matching Workshop.

==> body.tex <==



%%%%%%%%% Instructions
\section{Instructions}
% This section should be deleted when completed

\TODO{Remove this section for the final version.}
This document should provide just enough information for readers to reproduce
your outcomes. 
It also should list all datasets and pre-trained models for this purpose. This document should be shorter than 2 pages in length.

%%%%%%%%% BODY TEXT
\section{Method and Technical Details}

This section should discuss the technical details regarding your method. 
You should reference the method that was used, and provide any modifications that you performed to the method to achieve your performance.

In case you use your own RANSAC, please provide all RANSAC parameters as well. For example, the number of iterations would be important to make a fair comparison with other RANSAC methods.

SuperPoint 2k + SuperGlue

SuperPoint 4k + SuperGlue



\section{Dataset and Pre-trained Models}
We used the MegaDepth dataset with validation and test set removed to train our model from scratch.
